AgenticFinBench: Benchmarking Financial Agents on Diverse Tasks from Real-World Requests

Financial agents are becoming an important class of real-world AI systems. Financial tasks vary widely in type and difficulty, and many are open-ended with no ground-truth answers. However, existing benchmarks neither capture this breadth and open-endedness nor separate grounding from correctness. To bridge this gap, we introduce $\textbf{AgenticFinBench}$, a benchmark of 230 real-world financial tasks spanning 8 categories, 2 languages, and 4 complexity levels. We also propose a reference-free evaluation framework that combines question-specific rubrics with a two-stage claim audit that detects hallucinations, defined as claims absent from the agent's trace and refuted by external evidence. This framework better matches how financial work is assessed in practice. Experiments across 18 agent configurations reveal three key findings: (1) Ignoring hallucinations can overstate agent performance: hallucination auditing lowers the baseline leader's score by 7.58 points and moves it to fourth place. (2) Harness differences explain more variation in evidence grounding than model differences (28.6% vs 8.8%). (3) Quality scores fall from 89.44 on direct retrieval to 79.18 on the most complex tasks. Case studies show that agents struggle to explain how events affect company profits or stock prices, compare financial data on a consistent basis, and justify their conclusions. By releasing AgenticFinBench, we aim to advance financial reasoning, factual verification, and agent design for more reliable responses to diverse real-world financial requests.

==> tables/tab_ablation.tex <==
\begin{table}[!htbp]
\centering
\caption{Comparison using saved audit verdicts. \emph{Stage 1 only}: every ungrounded claim is called a hallucination. \emph{Stage 2 only}: every claim with a recorded external refutation is called a hallucination; external verdicts for grounded claims mostly reuse trace material, so this is an approximate comparison. Ordered by the Stage-1-only rate.}
\label{tab:ablation}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
Configuration & \makecell{Stage 1 only:\\``hallucination'' (\%)} & \makecell{of which externally\\verified (\%)} & \makecell{Stage 2 only:\\``hallucination'' (\%)} & \makecell{Two-stage\\hallucination (\%)} & \makecell{Unconfirmed\\$U$ (\%)} \\
\midrule

% Rows inlined for Overleaf compatibility; source snapshot: tables/tab_ablation_rows.tex
DeepSeek V4.1 Flash / Pi & 3.5 & 42.7 & 0.66 & 0.62 & 2.0 \\
DeepSeek V4.1 Flash / WorkBuddy & 6.8 & 60.5 & 1.41 & 0.92 & 2.7 \\
GPT-6 Luna / Codex CLI & 7.5 & 87.8 & 0.11 & 0.08 & 0.9 \\
DeepSeek V4.1 Flash / Codex CLI & 7.6 & 70.4 & 0.27 & 0.26 & 2.2 \\
GPT-6.1 Sol / Codex CLI & 8.4 & 90.5 & 0.07 & 0.07 & 0.8 \\
Claude Opus 5.5 / Pi & 14.3 & 85.2 & 0.27 & 0.20 & 2.1 \\
GPT-6 Astra / Codex CLI & 16.2 & 91.5 & 0.03 & 0.03 & 1.4 \\
Kimi K3 / Kimi hosted & 17.9 & 76.2 & 0.58 & 0.45 & 4.3 \\
GPT-5.6 Sol / Pi & 19.0 & 81.4 & 0.11 & 0.06 & 3.5 \\
GPT-5.6 Sol / Codex CLI & 19.7 & 87.3 & 0.10 & 0.09 & 2.5 \\
Gemini 4 Argon / Gemini CLI & 20.1 & 66.8 & 0.42 & 0.23 & 6.7 \\
Claude Opus 5.5 / Codex CLI & 20.5 & 84.5 & 0.51 & 0.40 & 3.2 \\
DeepSeek V4.1 Flash / DSH & 23.8 & 72.4 & 0.66 & 0.61 & 6.6 \\
Claude Opus 5.5 / Claude Code CLI & 29.8 & 87.6 & 0.71 & 0.40 & 3.7 \\
GPT-5.6 Sol / DSH & 41.7 & 83.9 & 0.32 & 0.31 & 6.7 \\
Claude Opus 5.5 / DSH & 56.3 & 83.3 & 0.87 & 0.80 & 9.4 \\
DuMate / DuMate CLI & 87.8 & 70.7 & 2.61 & 2.38 & 25.8 \\
Seed-2.1-pro / Trae Work & 99.0 & 71.6 & 2.13 & 2.13 & 28.1 \\

\bottomrule
\end{tabular}}
\end{table}


==> tables/tab_ablation_rows.tex <==
DeepSeek V4.1 Flash / Pi & 3.5 & 42.7 & 0.66 & 0.62 & 2.0 \\
DeepSeek V4.1 Flash / WorkBuddy & 6.8 & 60.5 & 1.41 & 0.92 & 2.7 \\
GPT-6 Luna / Codex CLI & 7.5 & 87.8 & 0.11 & 0.08 & 0.9 \\
DeepSeek V4.1 Flash / Codex CLI & 7.6 & 70.4 & 0.27 & 0.26 & 2.2 \\
GPT-6.1 Sol / Codex CLI & 8.4 & 90.5 & 0.07 & 0.07 & 0.8 \\
Claude Opus 5.5 / Pi & 14.3 & 85.2 & 0.27 & 0.20 & 2.1 \\
GPT-6 Astra / Codex CLI & 16.2 & 91.5 & 0.03 & 0.03 & 1.4 \\
Kimi K3 / Kimi hosted & 17.9 & 76.2 & 0.58 & 0.45 & 4.3 \\
GPT-5.6 Sol / Pi & 19.0 & 81.4 & 0.11 & 0.06 & 3.5 \\
GPT-5.6 Sol / Codex CLI & 19.7 & 87.3 & 0.10 & 0.09 & 2.5 \\
Gemini 4 Argon / Gemini CLI & 20.1 & 66.8 & 0.42 & 0.23 & 6.7 \\
Claude Opus 5.5 / Codex CLI & 20.5 & 84.5 & 0.51 & 0.40 & 3.2 \\
DeepSeek V4.1 Flash / DSH & 23.8 & 72.4 & 0.66 & 0.61 & 6.6 \\
Claude Opus 5.5 / Claude Code CLI & 29.8 & 87.6 & 0.71 & 0.40 & 3.7 \\
GPT-5.6 Sol / DSH & 41.7 & 83.9 & 0.32 & 0.31 & 6.7 \\
Claude Opus 5.5 / DSH & 56.3 & 83.3 & 0.87 & 0.80 & 9.4 \\
DuMate / DuMate CLI & 87.8 & 70.7 & 2.61 & 2.38 & 25.8 \\
Seed-2.1-pro / Trae Work & 99.0 & 71.6 & 2.13 & 2.13 & 28.1 \\


==> tables/tab_audit_execution_rows.tex <==
Kimi K3 / Kimi hosted & E & 4 & 444 & 56 & 4 \\
GPT-6 Astra / Codex CLI & E & 4 & 471 & 29 & 3 \\
GPT-5.6 Sol / Codex CLI & E & 4 & 458 & 42 & 14 \\
GPT-6 Luna / Codex CLI & B & 1 & 486 & 14 & 2 \\
Claude Opus 5.5 / Claude Code CLI & E + R780 & 4 & 417 & 83 & 11 \\
DeepSeek V4.1 Flash / Pi & B & 1 & 346 & 154 & 12 \\
DeepSeek V4.1 Flash / DSH & B & -- & 413 & 87 & 7 \\


==> tables/tab_audit_fields_rows.tex <==
\texttt{case\_\allowbreak{}id} & string; question identifier. \\
\texttt{items} & array; one entry for every extracted claim. \\
\texttt{summary} & string; coverage, errors, and unresolved issues. \\
\texttt{limitations} & array of strings; limitations of the audit. \\
\texttt{items[].claim\_\allowbreak{}id} & string; unchanged extracted claim identifier. \\
\texttt{items[].claim\_\allowbreak{}text} & string; unchanged extracted claim text. \\
\texttt{items[].trace\_\allowbreak{}verdict} & supported / unsupported / incomplete; original trace verdict. \\
\texttt{items[].trace\_\allowbreak{}reason} & string; explanation of the trace verdict. \\
\texttt{items[].factual\_\allowbreak{}verdict} & supported / contradicted / unresolved; original factual verdict. \\
\texttt{items[].fact\_\allowbreak{}reason} & string; explanation of the factual verdict. \\
\texttt{items[].evidence\_\allowbreak{}basis} & string; the basis and scope of the evidence used. \\
\texttt{items[].extraction\_\allowbreak{}issue} & string; mismatch or ambiguity introduced by extraction, if any. \\
\texttt{items[].evidence} & array; evidence records for this claim. \\
\texttt{evidence[].kind} & trace\_\allowbreak{}tool / trace\_\allowbreak{}context / external / calculation. \\
\texttt{evidence[].location} & string; JSON pointer, URL, or calculation expression. \\
\texttt{evidence[].quote} & string; source excerpt or calculation result. \\
\texttt{evidence[].title} & string; source or evidence title. \\
\texttt{evidence[].supports} & trace / fact / both / context. \\


==> tables/tab_audit_full_rows.tex <==
GPT-6 Astra / Codex CLI & 7,380 & 32.1 & 0.9 {\scriptsize(0.0--2.2)} & 0.03 {\scriptsize(0.00--0.07)} & 1.36 & 1.38 & 14.78 {\scriptsize(11.22--18.71)} & 13.5 \\
GPT-6 Luna / Codex CLI & 6,340 & 27.6 & 1.7 {\scriptsize(0.4--3.5)} & 0.08 {\scriptsize(0.02--0.17)} & 0.84 & 0.91 & 6.56 {\scriptsize(4.51--8.89)} & 11.7 \\
GPT-6.1 Sol / Codex CLI & 8,174 & 35.5 & 2.6 {\scriptsize(0.9--4.8)} & 0.07 {\scriptsize(0.02--0.14)} & 0.72 & 0.80 & 7.60 {\scriptsize(5.60--9.74)} & 13.9 \\
GPT-5.6 Sol / Pi & 11,326 & 49.2 & 2.6 {\scriptsize(0.9--4.8)} & 0.06 {\scriptsize(0.02--0.13)} & 3.46 & 3.52 & 15.45 {\scriptsize(11.01--20.44)} & 24.8 \\
GPT-5.6 Sol / Codex CLI & 10,626 & 46.2 & 3.0 {\scriptsize(0.9--5.2)} & 0.09 {\scriptsize(0.03--0.17)} & 2.41 & 2.50 & 17.20 {\scriptsize(10.83--23.73)} & 26.5 \\
GPT-5.6 Sol / DSH & 10,711 & 46.6 & 7.4 {\scriptsize(4.3--10.9)} & 0.31 {\scriptsize(0.15--0.54)} & 6.40 & 6.70 & 34.97 {\scriptsize(28.32--41.62)} & 47.4 \\
Claude Opus 5.5 / Pi & 12,812 & 55.7 & 10.9 {\scriptsize(7.0--14.8)} & 0.20 {\scriptsize(0.13--0.27)} & 1.93 & 2.12 & 12.18 {\scriptsize(9.27--15.21)} & 40.4 \\
Gemini 4 Argon / Gemini CLI & 19,575 & 85.1 & 12.6 {\scriptsize(8.7--17.0)} & 0.23 {\scriptsize(0.14--0.34)} & 6.44 & 6.67 & 13.38 {\scriptsize(10.73--16.50)} & 69.6 \\
DeepSeek V4.1 Flash / Codex CLI & 16,160 & 70.3 & 13.0 {\scriptsize(9.1--17.4)} & 0.26 {\scriptsize(0.18--0.36)} & 1.98 & 2.24 & 5.33 {\scriptsize(3.70--7.03)} & 39.6 \\
Claude Opus 5.5 / Codex CLI & 11,361 & 49.4 & 13.5 {\scriptsize(9.1--18.3)} & 0.40 {\scriptsize(0.23--0.61)} & 2.78 & 3.18 & 17.28 {\scriptsize(13.64--20.87)} & 46.5 \\
Claude Opus 5.5 / Claude Code CLI & 12,874 & 56.0 & 16.5 {\scriptsize(11.7--21.7)} & 0.40 {\scriptsize(0.27--0.55)} & 3.29 & 3.69 & 26.11 {\scriptsize(21.42--30.59)} & 48.7 \\
Claude Opus 5.5 / DSH & 10,850 & 47.2 & 21.7 {\scriptsize(16.5--27.0)} & 0.80 {\scriptsize(0.58--1.04)} & 8.57 & 9.37 & 46.91 {\scriptsize(40.18--52.88)} & 65.2 \\
Kimi K3 / Kimi hosted & 16,771 & 72.9 & 22.2 {\scriptsize(16.5--27.8)} & 0.45 {\scriptsize(0.33--0.59)} & 3.80 & 4.25 & 13.65 {\scriptsize(10.49--17.10)} & 60.9 \\
DeepSeek V4.1 Flash / WorkBuddy & 9,568 & 41.6 & 27.4 {\scriptsize(21.7--33.0)} & 0.92 {\scriptsize(0.70--1.15)} & 1.77 & 2.69 & 4.11 {\scriptsize(2.67--5.78)} & 44.3 \\
DeepSeek V4.1 Flash / DSH & 18,847 & 81.9 & 31.3 {\scriptsize(25.2--37.8)} & 0.61 {\scriptsize(0.47--0.77)} & 5.98 & 6.59 & 17.25 {\scriptsize(13.14--21.76)} & 67.0 \\
DeepSeek V4.1 Flash / Pi & 29,156 & 126.8 & 41.7 {\scriptsize(35.2--48.7)} & 0.62 {\scriptsize(0.50--0.75)} & 1.37 & 1.98 & 1.48 {\scriptsize(1.08--1.97)} & 66.5 \\
DuMate / DuMate CLI & 8,891 & 38.7 & 41.7 {\scriptsize(35.2--48.3)} & 2.38 {\scriptsize(1.92--2.84)} & 23.37 & 25.76 & 62.03 {\scriptsize(57.67--66.05)} & 90.0 \\
Seed-2.1-pro / Trae Work & 11,276 & 49.0 & 47.0 {\scriptsize(40.0--53.0)} & 2.13 {\scriptsize(1.63--2.64)} & 26.00 & 28.13 & 70.91 {\scriptsize(66.98--74.73)} & 88.7 \\


==> tables/tab_behavior_rows.tex <==
GPT-5.6 Sol / Codex CLI & 7 & 7.0\% \\
DeepSeek V4.1 Flash / Codex CLI & 75 & 2.6\% \\
GPT-5.6 Sol / Pi & 19.5 & 15.2\% \\
DeepSeek V4.1 Flash / Pi & 20 & 0.4\% \\
GPT-6.1 Sol / Codex CLI & 5 & 0.4\% \\
GPT-6 Astra / Codex CLI & 3 & 1.3\% \\
Kimi K3 / Kimi hosted & 3 & 5.2\% \\
DeepSeek V4.1 Flash / DSH & 24 & 6.1\% \\
Gemini 4 Argon / Gemini CLI & 4 & 14.8\% \\
Claude Opus 5.5 / Pi & 3 & 5.7\% \\
Claude Opus 5.5 / Claude Code CLI & 7 & 9.6\% \\
GPT-5.6 Sol / DSH & 15 & 23.9\% \\
Claude Opus 5.5 / Codex CLI & 0 & 56.5\% \\
Claude Opus 5.5 / DSH & 1 & 33.0\% \\
GPT-6 Luna / Codex CLI & 4 & 1.3\% \\
Seed-2.1-pro / Trae Work & --- & --- \\
DeepSeek V4.1 Flash / WorkBuddy & 22 & 0.0\% \\
DuMate / DuMate CLI & --- & --- \\


==> tables/tab_difficulty_rows.tex <==
\textit{Questions} & \textit{49} & \textit{14} & \textit{18} & \textit{17} & \textit{62} & \textit{17} & \textit{38} & \textit{15} & & \textit{10} & \textit{70} & \textit{86} & \textit{64} \\
\midrule
GPT-5.6 Sol / Codex CLI & 90.35 & \textbf{95.71} & 87.19 & 91.23 & 90.13 & 85.94 & 88.02 & 82.26 & & 95.04 & 91.25 & 88.32 & \textbf{87.22} \\
DeepSeek V4.1 Flash / Codex CLI & 90.89 & 92.00 & 85.18 & 86.40 & \textbf{91.42} & 87.49 & 86.79 & 81.57 & & 88.07 & 90.83 & \textbf{88.91} & 86.49 \\
GPT-5.6 Sol / Pi & 90.07 & 94.28 & 85.93 & 85.85 & 90.23 & 85.90 & 87.28 & 84.85 & & 91.46 & 90.96 & 87.56 & 87.06 \\
DeepSeek V4.1 Flash / Pi & 93.76 & 93.72 & 87.78 & 83.82 & 84.06 & 86.29 & 87.78 & 85.17 & & \textbf{97.83} & \textbf{92.73} & 86.62 & 82.56 \\
GPT-6.1 Sol / Codex CLI & 88.48 & 88.28 & 83.14 & \textbf{91.40} & 88.15 & 86.79 & 89.30 & 80.75 & & 85.62 & 88.96 & 88.06 & 86.10 \\
GPT-6 Astra / Codex CLI & 88.82 & 92.74 & 84.09 & 88.09 & 88.04 & 86.50 & 85.40 & 82.38 & & 91.46 & 88.88 & 86.94 & 85.29 \\
Kimi K3 / Kimi hosted & 88.16 & 91.94 & \textbf{89.83} & 75.67 & 85.33 & \textbf{88.67} & \textbf{89.35} & 83.18 & & 93.12 & 88.04 & 86.45 & 84.72 \\
DeepSeek V4.1 Flash / DSH & \textbf{94.00} & 93.65 & 87.41 & 85.10 & 79.45 & 87.71 & 85.24 & 76.39 & & 96.28 & 91.65 & 87.16 & 76.03 \\
Gemini 4 Argon / Gemini CLI & 87.31 & 93.78 & 83.91 & 80.07 & 82.90 & 85.02 & 84.03 & \textbf{88.60} & & 88.21 & 89.41 & 84.15 & 81.13 \\
Claude Opus 5.5 / Pi & 89.28 & 89.65 & 84.71 & 78.45 & 85.76 & 85.86 & 80.06 & 81.67 & & 89.96 & 88.50 & 83.49 & 82.15 \\
Claude Opus 5.5 / Claude Code CLI & 92.51 & 91.02 & 75.60 & 84.93 & 80.24 & 85.83 & 83.34 & 79.65 & & 91.77 & 90.17 & 82.22 & 79.80 \\
GPT-5.6 Sol / DSH & 86.80 & 88.01 & 76.73 & 83.91 & 86.06 & 85.54 & 80.63 & 78.67 & & 82.34 & 85.96 & 83.62 & 82.73 \\
Claude Opus 5.5 / Codex CLI & 87.37 & 92.00 & 80.20 & 76.89 & 82.05 & 83.01 & 82.00 & 79.04 & & 90.71 & 87.48 & 82.09 & 78.58 \\
Claude Opus 5.5 / DSH & 85.76 & 83.65 & 81.70 & 80.26 & 78.51 & 84.33 & 77.71 & 72.86 & & 81.68 & 85.03 & 78.29 & 78.97 \\
GPT-6 Luna / Codex CLI & 75.21 & 85.35 & 75.63 & 79.50 & 79.44 & 79.08 & 80.91 & 77.46 & & 73.54 & 80.11 & 78.43 & 78.30 \\
Seed-2.1-pro / Trae Work & 87.71 & 93.82 & 74.40 & 75.63 & 67.26 & 70.50 & 85.57 & 71.47 & & 91.80 & 86.07 & 78.72 & 65.87 \\
DeepSeek V4.1 Flash / WorkBuddy & 75.43 & 91.52 & 76.06 & 71.87 & 68.03 & 69.59 & 63.12 & 68.36 & & 95.72 & 78.93 & 70.07 & 60.70 \\
DuMate / DuMate CLI & 65.40 & 76.41 & 53.57 & 60.36 & 58.39 & 77.31 & 75.43 & 65.41 & & 85.21 & 65.29 & 66.17 & 61.48 \\
\midrule
Mean of 18 & 86.52 & 90.42 & 80.72 & 81.08 & 81.41 & 83.41 & 82.89 & 78.88 & & 89.44 & 86.68 & 82.63 & 79.18 \\


==> tables/tab_extraction_fields_rows.tex <==
\texttt{claim\_\allowbreak{}id} & string & Unique claim identifier, ordered within the response. \\
\texttt{claim\_\allowbreak{}text} & string & Standalone factual proposition preserving material qualifiers. \\
\texttt{claim\_\allowbreak{}type} & enum & Our extraction prompt permits numeric\_\allowbreak{}fact, derived\_\allowbreak{}numeric, event\_\allowbreak{}fact, source\_\allowbreak{}attribution, or mechanism\_\allowbreak{}statement. \\
\texttt{subject} & object or null & Entity: name plus optional ticker, market, and entity\_\allowbreak{}id. Required for numeric claims. \\
\texttt{predicate\_\allowbreak{}or\_\allowbreak{}metric} & string or null & Property or metric asserted about the subject; required for numeric claims. \\
\texttt{value} & JSON value or null & Asserted value; required for numeric claims. \\
\texttt{unit} & string or null & Measurement unit when stated in the response. \\
\texttt{currency} & string or null & Currency when stated in the response. \\
\texttt{financial\_\allowbreak{}period} & string or null & Reporting period when stated in the response. \\
\texttt{as\_\allowbreak{}of} & datetime or null & Temporal qualifier when stated; not an added question requirement. \\
\texttt{source\_\allowbreak{}attribution} & string or null & Source attribution stated in the response, if any. \\
\texttt{answer\_\allowbreak{}span} & object & unit\_\allowbreak{}id identifies the answer unit; start and end are global character offsets. The intended span is the smallest supporting span within that unit. \\
\texttt{is\_\allowbreak{}key\_\allowbreak{}claim} & boolean & Key-claim flag emitted by the extractor; not a truth judgment. \\
\texttt{verifiability} & enum & Schema values: deterministic, semantic, not\_\allowbreak{}verifiable. Our extraction prompt excludes non-factual claims. \\
\texttt{enters\_\allowbreak{}factual\_\allowbreak{}denominator} & boolean & Whether the claim enters the factual denominator; our extraction prompt requires true for every extracted claim. \\


==> tables/tab_main.tex <==
\centering
\captionof{table}{Quality results for 18 configurations on the same 230 questions. $Q$ is the quality score and $B$ is the baseline score, both on a 0--100 scale. Intervals are 95\% paired question-bootstrap intervals from 10,000 resamples. Rows and ranks use mean point estimates; adjacent ranks need not differ significantly.}
\label{tab:main}
\small
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}rlrrrc@{}}
\toprule
Rank & Agent configuration & {\boldmath$Q$} & 95\% CI & $Q-B$ & \makecell{Rank\\$B\to Q$} \\
\midrule

% Rows inlined for Overleaf compatibility; source snapshot: tables/tab_main_rows.tex
1 & GPT-5.6 Sol / Codex CLI & \textbf{89.20} & 87.61--90.71 & -0.27 & 5 $\rightarrow$ 1 \\
2 & DeepSeek V4.1 Flash / Codex CLI & \textbf{88.79} & 87.44--90.09 & -1.46 & 2 $\rightarrow$ 2 \\
3 & GPT-5.6 Sol / Pi & \textbf{88.62} & 87.31--89.89 & -0.38 & 6 $\rightarrow$ 3 \\
4 & DeepSeek V4.1 Flash / Pi & \textbf{87.84} & 85.87--89.64 & -7.58 & 1 $\rightarrow$ 4 \\
5 & GPT-6.1 Sol / Codex CLI & \textbf{87.68} & 85.98--89.31 & -0.13 & 7 $\rightarrow$ 5 \\
6 & GPT-6 Astra / Codex CLI & \textbf{87.27} & 85.69--88.84 & -0.01 & 9 $\rightarrow$ 6 \\
7 & Kimi K3 / Kimi hosted & \textbf{86.74} & 84.39--88.87 & -3.46 & 3 $\rightarrow$ 7 \\
8 & DeepSeek V4.1 Flash / DSH & \textbf{85.82} & 83.67--87.87 & -3.87 & 4 $\rightarrow$ 8 \\
9 & Gemini 4 Argon / Gemini CLI & \textbf{85.09} & 83.32--86.79 & -2.54 & 8 $\rightarrow$ 9 \\
10 & Claude Opus 5.5 / Pi & \textbf{84.92} & 83.47--86.39 & -0.99 & 11 $\rightarrow$ 10 \\
11 & Claude Opus 5.5 / Claude Code CLI & \textbf{84.38} & 82.56--86.17 & -2.54 & 10 $\rightarrow$ 11 \\
12 & GPT-5.6 Sol / DSH & \textbf{84.03} & 82.11--85.84 & -1.41 & 12 $\rightarrow$ 12 \\
13 & Claude Opus 5.5 / Codex CLI & \textbf{83.13} & 81.40--84.80 & -1.30 & 13 $\rightarrow$ 13 \\
14 & Claude Opus 5.5 / DSH & \textbf{80.68} & 78.77--82.50 & -3.08 & 14 $\rightarrow$ 14 \\
15 & GPT-6 Luna / Codex CLI & \textbf{78.69} & 76.74--80.67 & -0.20 & 16 $\rightarrow$ 15 \\
16 & Seed-2.1-pro / Trae Work & \textbf{77.95} & 74.69--80.99 & -3.44 & 15 $\rightarrow$ 16 \\
17 & DeepSeek V4.1 Flash / WorkBuddy & \textbf{71.27} & 68.39--74.09 & -3.90 & 17 $\rightarrow$ 17 \\
18 & DuMate / DuMate CLI & \textbf{65.42} & 62.43--68.32 & -5.44 & 18 $\rightarrow$ 18 \\

\bottomrule
\end{tabular}%
}


==> tables/tab_main_rows.tex <==
1 & GPT-5.6 Sol / Codex CLI & \textbf{89.20} & 87.61--90.71 & 89.47 & -0.27 & 5 $\rightarrow$ 1 \\
2 & DeepSeek V4.1 Flash / Codex CLI & \textbf{88.79} & 87.44--90.09 & 90.24 & -1.46 & 2 $\rightarrow$ 2 \\
3 & GPT-5.6 Sol / Pi & \textbf{88.62} & 87.31--89.89 & 89.00 & -0.38 & 6 $\rightarrow$ 3 \\
4 & DeepSeek V4.1 Flash / Pi & \textbf{87.84} & 85.87--89.64 & 95.42 & -7.58 & 1 $\rightarrow$ 4 \\
5 & GPT-6.1 Sol / Codex CLI & \textbf{87.68} & 85.98--89.31 & 87.81 & -0.13 & 7 $\rightarrow$ 5 \\
6 & GPT-6 Astra / Codex CLI & \textbf{87.27} & 85.69--88.84 & 87.28 & -0.01 & 9 $\rightarrow$ 6 \\
7 & Kimi K3 / Kimi hosted & \textbf{86.74} & 84.39--88.87 & 90.21 & -3.46 & 3 $\rightarrow$ 7 \\
8 & DeepSeek V4.1 Flash / DSH & \textbf{85.82} & 83.67--87.87 & 89.69 & -3.87 & 4 $\rightarrow$ 8 \\
9 & Gemini 4 Argon / Gemini CLI & \textbf{85.09} & 83.32--86.79 & 87.63 & -2.54 & 8 $\rightarrow$ 9 \\
10 & Claude Opus 5.5 / Pi & \textbf{84.92} & 83.47--86.39 & 85.91 & -0.99 & 11 $\rightarrow$ 10 \\
11 & Claude Opus 5.5 / Claude Code CLI & \textbf{84.38} & 82.56--86.17 & 86.92 & -2.54 & 10 $\rightarrow$ 11 \\
12 & GPT-5.6 Sol / DSH & \textbf{84.03} & 82.11--85.84 & 85.44 & -1.41 & 12 $\rightarrow$ 12 \\
13 & Claude Opus 5.5 / Codex CLI & \textbf{83.13} & 81.40--84.80 & 84.43 & -1.30 & 13 $\rightarrow$ 13 \\
14 & Claude Opus 5.5 / DSH & \textbf{80.68} & 78.77--82.50 & 83.76 & -3.08 & 14 $\rightarrow$ 14 \\
15 & GPT-6 Luna / Codex CLI & \textbf{78.69} & 76.74--80.67 & 78.89 & -0.20 & 16 $\rightarrow$ 15 \\
16 & Seed-2.1-pro / Trae Work & \textbf{77.95} & 74.69--80.99 & 81.39 & -3.44 & 15 $\rightarrow$ 16 \\
17 & DeepSeek V4.1 Flash / WorkBuddy & \textbf{71.27} & 68.39--74.09 & 75.18 & -3.90 & 17 $\rightarrow$ 17 \\
18 & DuMate / DuMate CLI & \textbf{65.42} & 62.43--68.32 & 70.87 & -5.44 & 18 $\rightarrow$ 18 \\


==> tables/tab_paired_rows.tex <==
GPT-6 Luna $-$ GPT-6 Astra & [-0.9, +3.0] & [-0.03, +0.14] & [-11.0, -5.6]$^{*}$ \\
GPT-6.1 Sol $-$ GPT-6 Luna & [-1.7, +3.5] & [-0.11, +0.09] & [-1.2, +3.2] \\
Sol 5.6 / Pi $-$ GPT-6.1 Sol & [-3.0, +3.0] & [-0.09, +0.07] & [+3.9, +12.2]$^{*}$ \\
GPT-5.6 Sol $-$ Sol 5.6 / Pi & [-2.6, +3.5] & [-0.06, +0.13] & [-3.1, +7.6] \\
Sol 5.6 / DSH $-$ GPT-5.6 Sol & [+0.4, +8.7]$^{*}$ & [+0.03, +0.44]$^{*}$ & [+11.1, +24.1]$^{*}$ \\
Opus 5.5 / Pi $-$ Sol 5.6 / DSH & [-1.7, +8.7] & [-0.35, +0.07] & [-28.2, -17.7]$^{*}$ \\
Gemini 4 / Gemini $-$ Opus 5.5 / Pi & [-3.9, +7.4] & [-0.09, +0.17] & [-1.6, +4.0] \\
DS-V4.1 / Codex $-$ Gemini 4 / Gemini & [-5.7, +6.1] & [-0.12, +0.17] & [-10.5, -5.8]$^{*}$ \\
Opus 5.5 / Codex $-$ DS-V4.1 / Codex & [-5.7, +6.1] & [-0.05, +0.36] & [+8.8, +15.3]$^{*}$ \\
Opus 5.5 $-$ Opus 5.5 / Codex & [-3.5, +9.1] & [-0.24, +0.20] & [+5.8, +11.7]$^{*}$ \\
Opus 5.5 / DSH $-$ Opus 5.5 & [-1.7, +12.2] & [+0.17, +0.67]$^{*}$ & [+16.0, +26.4]$^{*}$ \\
Kimi K3 $-$ Opus 5.5 / DSH & [-7.8, +8.7] & [-0.66, -0.06]$^{*}$ & [-39.7, -27.2]$^{*}$ \\
DS-V4.1 / WorkBuddy $-$ Kimi K3 & [-2.6, +12.6] & [+0.22, +0.74]$^{*}$ & [-12.8, -6.6]$^{*}$ \\
DS-V4.1 / DSH $-$ DS-V4.1 / WorkBuddy & [-4.8, +12.2] & [-0.58, -0.04]$^{*}$ & [+9.5, +17.5]$^{*}$ \\
DS-V4.1 / Pi $-$ DS-V4.1 / DSH & [+2.2, +18.7]$^{*}$ & [-0.20, +0.20] & [-20.4, -12.1]$^{*}$ \\
DuMate $-$ DS-V4.1 / Pi & [-8.7, +8.7] & [+1.31, +2.28]$^{*}$ & [+56.3, +64.7]$^{*}$ \\
Seed-2.1 / Trae $-$ DuMate & [-3.0, +13.9] & [-0.89, +0.43] & [+3.6, +13.9]$^{*}$ \\


==> tables/tab_question_examples.tex <==
\begin{table}[!htbp]
\centering
\caption{Illustrative questions from the frozen dataset. Chinese originals are followed by English translations in gray; English originals are reproduced as written. ZH / EN indicates the original language. The purposive selection illustrates variety, not category frequencies.}
\label{tab:question-examples}
\small
% \setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.8}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{2.25cm}>{\raggedright\arraybackslash}Xc@{}}
\toprule
ID & Question & Language \\
\midrule

% Rows inlined for Overleaf compatibility; source snapshot: tables/tab_question_examples_rows.tex
prod100-008 & 请问纳斯达克100 和qqq 两个是不同的ETF吗？\newline{\color{black!65}Are the Nasdaq 100 and QQQ two different ETFs?} & ZH \\[5pt]
prod386-098 & 2026/7/31中美10年国债收益率分别是多少？\newline{\color{black!65}What were the yields on 10-year Chinese and US government bonds on July 31, 2026?} & ZH \\[5pt]
prod100-049 & 2025年离岸央票有没有用来维稳汇率？有没有引起离岸利率提高？\newline{\color{black!65}Were offshore central bank bills used to stabilize the exchange rate in 2025? Did they raise offshore interest rates?} & ZH \\[5pt]
prod100-010 & 说下你对行业的分析框架，可以举例的方向。比如你怎么看低温奶行业。\newline{\color{black!65}Describe your framework for industry analysis, with an example. For instance, how do you view the chilled milk industry?} & ZH \\[5pt]
prod100-072 & 综合各维度比较一下胜宏科技和沪电股份，给出投资建议\newline{\color{black!65}Compare Victory Giant Technology and Wus Printed Circuit across dimensions and provide investment advice.} & ZH \\[5pt]
prod386-360 & 生产一篇三一重工的投研分析报告，重点分析企业的劣势和风险。\newline{\color{black!65}Produce an investment research report on Sany Heavy Industry, focusing on its weaknesses and risks.} & ZH \\[5pt]
prod386-330 & 你如何看待科创50后续的走势？我希望能构建一个稳健的指数投资策略，你的建议是什么？\newline{\color{black!65}How do you view the future trend of the STAR 50? I would like to build a robust index investment strategy. What would you recommend?} & ZH \\[5pt]
prod386-364 & 如果 AI 行业盈利预期长期没有改善，对于黄金的影响是什么？\newline{\color{black!65}If earnings expectations for the AI industry do not improve over the long term, what would the impact on gold be?} & ZH \\[5pt]
en120-001 & Analyze Nvidia and create a research report for me. & EN \\[5pt]
en120-005 & What is the institutional consensus on SK hynix in recent research, and where do analysts disagree? & EN \\[5pt]
en120-011 & Why charter hall’s deal and performance fees dry up when the cost of capital is high? & EN \\[5pt]
en120-120 & What’s chapter 2 of the intelligent investor saying??? & EN \\[5pt]


\bottomrule
\end{tabularx}
\end{table}


==> tables/tab_question_examples_rows.tex <==
prod100-008 & 请问纳斯达克100 和qqq 两个是不同的ETF吗？\newline{\color{black!65}Are the Nasdaq 100 and QQQ two different ETFs?} & ZH \\[5pt]
prod386-098 & 2026/7/31中美10年国债收益率分别是多少？\newline{\color{black!65}What were the yields on 10-year Chinese and US government bonds on July 31, 2026?} & ZH \\[5pt]
prod100-049 & 2025年离岸央票有没有用来维稳汇率？有没有引起离岸利率提高？\newline{\color{black!65}Were offshore central bank bills used to stabilize the exchange rate in 2025? Did they raise offshore interest rates?} & ZH \\[5pt]
prod100-010 & 说下你对行业的分析框架，可以举例的方向。比如你怎么看低温奶行业。\newline{\color{black!65}Describe your framework for industry analysis, with an example. For instance, how do you view the chilled milk industry?} & ZH \\[5pt]
prod100-072 & 综合各维度比较一下胜宏科技和沪电股份，给出投资建议\newline{\color{black!65}Compare Victory Giant Technology and Wus Printed Circuit across dimensions and provide investment advice.} & ZH \\[5pt]
prod386-360 & 生产一篇三一重工的投研分析报告，重点分析企业的劣势和风险。\newline{\color{black!65}Produce an investment research report on Sany Heavy Industry, focusing on its weaknesses and risks.} & ZH \\[5pt]
prod386-330 & 你如何看待科创50后续的走势？我希望能构建一个稳健的指数投资策略，你的建议是什么？\newline{\color{black!65}How do you view the future trend of the STAR 50? I would like to build a robust index investment strategy. What would you recommend?} & ZH \\[5pt]
prod386-364 & 如果 AI 行业盈利预期长期没有改善，对于黄金的影响是什么？\newline{\color{black!65}If earnings expectations for the AI industry do not improve over the long term, what would the impact on gold be?} & ZH \\[5pt]
en120-001 & Analyze Nvidia and create a research report for me. & EN \\[5pt]
en120-005 & What is the institutional consensus on SK hynix in recent research, and where do analysts disagree? & EN \\[5pt]
en120-011 & Why charter hall’s deal and performance fees dry up when the cost of capital is high? & EN \\[5pt]
en120-120 & What’s chapter 2 of the intelligent investor saying??? & EN \\[5pt]


==> tables/tab_rubric_negative_rows.tex <==
N01 & Asserts that if PE stops rising, the share price definitely cannot rise, ignoring EPS growth, buybacks, or other factors. Statements such as ``it may not rise'' or ``it is hard to rise without earnings growth,'' or a discussion of risks alone, do not trigger this item. & 80; cap 20 \\[5pt]
N02 & Defines PE as earnings per share divided by the share price (or net profit divided by market capitalization), inverting numerator and denominator. Merely noting that PE can be negative does not trigger this item. & 25; cap 60 \\[5pt]
N03 & Asserts that a rising PE necessarily raises the share price or a falling PE necessarily lowers it, treating changes in the multiple as necessary and sufficient for price changes. Discussing what usually or may happen does not trigger this item. & 12 \\[5pt]
N04 & Cites a specific Nvidia PE or share price without any date or basis and presents it as a current or long-term fact. Figures explicitly labeled as examples or assumptions do not trigger this item. & 12 \\[5pt]
N05 & Promises or guarantees that Nvidia's share price will still rise if PE stops rising, presenting a possibility as a certain gain. A conditional scenario alone does not trigger this item. & 25; cap 60 \\[5pt]
N06 & Compares Nvidia's TTM and forward PE interchangeably without stating the basis and draws a definite valuation conclusion from the comparison. Merely listing both does not trigger this item. & 12 \\[5pt]
N07 & Multiplies one quarter's earnings by four, calls the result actual full-year earnings without labeling the annualization assumption, and computes PE from it. An explicitly labeled annualization assumption does not trigger this item. & 12 \\[5pt]
N08 & Equates a high PE with a high share price or with certain overvaluation or a bubble, ignoring differences in growth and risk. Discussing possibilities or conditions does not trigger this item. & 12 \\[5pt]


==> tables/tab_stats.tex <==
% Retained source snapshot; superseded in the manuscript by fig_dataset_overview.pdf.
% Table half of the side-by-side float with fig:distribution (Section 3.1); rows from scripts/make_distribution.py.
% Run-level counts (11 configurations, 2,530 responses, 139,903 claims, 27.6--126.8 claims per response)
% are reported in Section 5.1 and Appendix I.
\captionof{table}{Dataset statistics.}
\label{tab:stats}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X r@{}}
\toprule
\textbf{Statistic} & \textbf{Value} \\
\midrule

% Rows inlined for Overleaf compatibility; source snapshot: tables/tab_stats_rows.tex
% Generated by scripts/make_distribution.py; do not edit by hand.
\textbf{Questions} & \\
\quad Total & 230 \\
\quad Chinese / English & 189 / 41 \\
\quad Seed / expansion / English batch & 44 / 146 / 40 \\
\midrule
\textbf{Length, median} & \\
\quad Chinese (characters) & 25 \\
\quad English (words) & 56 \\
\midrule
\textbf{Taxonomy} & \\
\quad Categories & 8 \\
\quad Complexity L1 / L2 / L3 / L4 & 10 / 70 / 86 / 64 \\
\midrule
\textbf{Rubrics} & \\
\quad Items, positive / negative & 5,817 / 1,780 \\
\quad Per question, median (range) & 35 (13--47) \\
\quad Per question, median pos. / neg. & 27 / 8 \\

\bottomrule
\end{tabularx}

% \vspace{3pt}
% {\raggedright\sffamily\fontsize{7.6}{10.2}\selectfont\color{nnSecondary}
% $^\dagger$Eight categories cover all 230 questions; each question has one primary category based on its requested deliverable.
% $^\ddagger$Agent-reviewed labels under the revised definitions in \cref{tab:task-complexity}; expert review remains pending.\par}


==> tables/tab_stats_rows.tex <==
% Generated by scripts/make_distribution.py; do not edit by hand.
\textbf{Questions} & \\
\quad Total & 230 \\
\quad Chinese / English & 189 / 41 \\
\quad Seed / expansion / English batch & 44 / 146 / 40 \\
\midrule
\textbf{Length, median} & \\
\quad Chinese (characters) & 25 \\
\quad English (words) & 56 \\
\midrule
\textbf{Taxonomy} & \\
\quad Categories & 8 \\
\quad Complexity L1 / L2 / L3 / L4 & 10 / 70 / 86 / 64 \\
\midrule
\textbf{Rubrics} & \\
\quad Items, positive / negative & 5,817 / 1,780 \\
\quad Per question, median (range) & 35 (13--47) \\
\quad Per question, median pos. / neg. & 27 / 8 \\


==> tables/tab_structure_rows.tex <==
GPT-6 Astra / Codex CLI & 83.83 & 53.9 & 9.6 & 1.3 & 1.65 & 92 & 0.2 & 0 \\
GPT-6 Luna / Codex CLI & 92.52 & 31.3 & 5.7 & 1.3 & 1.02 & 93 & 1.2 & 2 \\
GPT-6.1 Sol / Codex CLI & 91.61 & 41.7 & 3.5 & 0.4 & 0.93 & 86 & 1.0 & 0 \\
GPT-5.6 Sol / Pi & 81.03 & 49.6 & 15.2 & 14.8 & 2.65 & 89 & 0.4 & 6 \\
GPT-5.6 Sol / Codex CLI & 80.29 & 55.7 & 13.0 & 7.0 & 2.26 & 80 & 0.5 & 1 \\
GPT-5.6 Sol / DSH & 58.32 & 73.5 & 52.2 & 44.3 & 6.99 & 65 & 0.9 & 1 \\
Claude Opus 5.5 / Pi & 85.70 & 65.2 & 11.7 & 4.3 & 2.51 & 64 & 1.6 & 9 \\
Gemini 4 Argon / Gemini CLI & 79.95 & 80.0 & 20.9 & 14.8 & 7.29 & 56 & 1.7 & 38 \\
DeepSeek V4.1 Flash / Codex CLI & 92.43 & 49.6 & 6.5 & 4.3 & 2.52 & 67 & 4.6 & 1 \\
Claude Opus 5.5 / Codex CLI & 79.54 & 67.0 & 18.3 & 8.3 & 3.31 & 59 & 2.2 & 13 \\
Claude Opus 5.5 / Claude Code CLI & 70.20 & 82.6 & 30.0 & 8.3 & 3.44 & 62 & 1.5 & 40 \\
Claude Opus 5.5 / DSH & 43.71 & 93.0 & 69.1 & 58.7 & 11.10 & 52 & 1.7 & 7 \\
Kimi K3 / Kimi hosted & 82.10 & 72.2 & 13.5 & 5.2 & 4.10 & 62 & 3.2 & 23 \\
DeepSeek V4.1 Flash / WorkBuddy & 93.21 & 28.7 & 3.5 & 0.4 & 2.79 & 52 & 18.3 & 47 \\
DeepSeek V4.1 Flash / DSH & 76.16 & 72.6 & 30.4 & 20.9 & 7.73 & 60 & 3.4 & 10 \\
DeepSeek V4.1 Flash / Pi & 96.54 & 50.0 & 0.9 & 0.4 & 2.03 & 48 & 29.5 & 13 \\
DuMate / DuMate CLI & 12.21 & 97.4 & 90.4 & 59.1 & 23.89 & 38 & 3.7 & 20 \\
Seed-2.1-pro / Trae Work & 0.96 & 98.7 & 100.0 & 88.3 & 27.28 & 39 & 2.9 & 0 \\


==> tables/tab_task_complexity.tex <==
\begin{table}[H]
\centering
\caption{Task complexity levels, defined by the required information synthesis and decision autonomy. Examples are illustrative; levels do not measure empirical difficulty.}
\label{tab:task-complexity}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.18}
\begin{tabularx}{\textwidth}{@{}l >{\raggedright\arraybackslash}p{2.55cm} >{\hsize=1.15\hsize\raggedright\arraybackslash}X >{\hsize=.85\hsize\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Level} & \textbf{Category} & \textbf{Required work} & \textbf{Illustrative query} \\
\midrule
\textbf{L1} & Direct retrieval
& Retrieve a single fact, existing record, basic definition, or explicit rule, without organizing multiple information dimensions or choosing an analytical method.
& What is a gold ETF? What is the current gold price? \\
\addlinespace[5pt]
\textbf{L2} & Structured synthesis
& Organize information, perform standard calculations, screening or comparisons, or explain established mechanisms and procedures, without independent investment judgment.
& Compare the returns and maximum drawdowns of gold and the S\&P 500 over the past year. \\
\addlinespace[5pt]
\textbf{L3} & Focused analysis
& Use evidence to explain causes, diagnose a problem, or judge a specific issue, without requiring a comprehensive investment thesis or a self-designed model or plan.
& Why did the company's gross margin decline in its latest financial report? \\
\addlinespace[5pt]
\textbf{L4} & Research and decision design
& Choose an analytical framework and integrate complementary factors to develop a comprehensive investment thesis, weigh forward-looking investment choices, or design and evaluate a model or plan under assumptions, constraints, and uncertainty.
& Develop an investment thesis integrating the company's business, industry, valuation, and risks, and identify conditions that would invalidate it. \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/tab_taxonomy_category_rows.tex <==
Knowledge Q\&A & Explain financial concepts, product mechanisms, trading rules or general research methods. & 49 & 21.3 \\
Data \& calculation & Retrieve facts or documents, organize data, or perform specified calculations without an investment conclusion. & 14 & 6.1 \\
Screening & Find securities or investment products in an open candidate universe that match stated criteria. & 18 & 7.8 \\
Comparison & Compare specified securities or products and, where requested, choose among them. & 17 & 7.4 \\
Investment research & Develop an integrated assessment of a company, sector, market or asset, including prospects, value and risks. & 62 & 27.0 \\
Financial analysis & Interpret financial disclosures, operating results, earnings quality, cash flows or management guidance. & 17 & 7.4 \\
Event analysis & Assess the market effects of a specific news event, policy action, data release or explicit shock scenario. & 38 & 16.5 \\
Investment planning & Value or forecast assets, diagnose or allocate portfolios, or design and validate investment strategies. & 15 & 6.5 \\


==> tables/tab_taxonomy_level_rows.tex <==
% Generated by scripts/make_distribution.py; do not edit by hand.
\textbf{L1}\newline Direct retrieval & Retrieve a single fact, existing record, basic definition, or explicit rule, without organizing multiple information dimensions or choosing an analytical method. & Are the Nasdaq 100 and QQQ two different ETFs? {\color{nnSecondary}\footnotesize (ZH)}  \\
\addlinespace[3pt]
\textbf{L2}\newline Structured synthesis & Organize information, perform standard calculations, screening or comparisons, or explain established mechanisms and procedures, without independent investment judgment. & Which US-listed companies are involved in edge AI? {\color{nnSecondary}\footnotesize (ZH)}  \\
\addlinespace[3pt]
\textbf{L3}\newline Focused analysis & Use evidence to explain causes, diagnose a problem, or judge a specific issue, without requiring a comprehensive investment thesis or a self-designed model or plan. & Historically, has AMD's guidance tended to be conservative or optimistic? {\color{nnSecondary}\footnotesize (ZH)}  \\
\addlinespace[3pt]
\textbf{L4}\newline Research and decision design & Choose an analytical framework and integrate complementary factors to develop a comprehensive investment thesis, weigh forward-looking investment choices, or design and evaluate a model or plan under assumptions, constraints, and uncertainty. & Do a DCF valuation of Haitian Flavouring and Food. {\color{nnSecondary}\footnotesize (ZH)}  \\

